Recursive Mechanism: Towards Node Differential Privacy and Unrestricted Joins [Full Version, Draft 0.1]

Existing studies on differential privacy mainly consider aggregation on data sets where each entry corresponds to a particular participant to be protected. In many situations, a user may pose a relational algebra query on a sensitive database, and desires differentially private aggregation on the result of the query. However, no known work is capable to release this kind of aggregation when the query contains unrestricted join operations. This severely limits the applications of existing differential privacy techniques because many data analysis tasks require unrestricted joins. One example is subgraph counting on a graph. Existing methods for differentially private subgraph counting address only edge differential privacy and are subject to very simple subgraphs. Before this work, whether any nontrivial graph statistics can be released with reasonable accuracy under node differential privacy is still an open problem. In this paper, we propose a novel differentially private mechanism to release an approximation to a linear statistic of the result of some positive relational algebra calculation over a sensitive database. Unrestricted joins are supported in our mechanism. The error bound of the approximate answer is roughly proportional to the \emph{empirical sensitivity} of the query --- a new notion that measures the maximum possible change to the query answer when a participant withdraws its data from the sensitive database. For subgraph counting, our mechanism provides the first solution to achieve node differential privacy, for any kind of subgraphs.

==> intro.tex <==
\section{Introduction}\label{sec:intro}

An important task in data privacy research is to develop mechanisms to publish useful results mined from sensitive database, without disclosing individual privacy. Most of existing techniques provide rather limited privacy protection, since they often address specific attack models, or rely on specific assumptions about the prior knowledge the potential adversary may possess. In recent years, the paradigm of differential privacy has received increasing attention, since it can provide robust and quantitative privacy guarantee while making no assumptions about the prior knowledge of the adversary. Data publishing algorithms that achieve differential privacy should guarantee that their output are randomized such that input databases differing in one participant are almost indistinguishable to the adversary. Therefore, participating in a database is unlikely to cause privacy breach.

Existing studies on differential privacy often address a simple data model, where the input database is a set of records, and each record corresponds to a participant. The output of a differentially private data publishing algorithm should have almost identical probability distributions for input data sets that differ in exactly one record. Then, various kinds of queries that compute aggregations on data sets are considered. Much effort has been put to linear aggregations, on which more complex queries can be built.

The success of most existing differentially private mechanisms relies on the precondition that the maximum possible change to the query answer resulted from the change of one participant should be small and bounded. Such maximum possible change is called the \emph{sensitivity} of the query, which determines the minimum magnitude of noise needed to introduce into the answer. In practice, however, many databases contain information about not only individual participants, but also relationships between them. The change of one participant may, in the worst case, have potentially unlimited impact on the database and the query answer. Queries on such databases are too complex to be tackled by existing techniques. In this paper, we try to relax the precondition by allowing potentially unbounded impact that could be incurred by new participants joining the database, and give an elegant solution.

\subsection{Motivation}

Subgraph counting is an important problem in data mining and social networks, which counts the number of occurrences of a given query subgraph in an input graph. Despite of the enormous work on anonymization schemes for private graphs, little has been down to provide quantitative guarantees of privacy and utility. In~\cite{DBLP:conf/pods/RastogiHMS09}, subgraph counting is studied under a much weaker version of differential privacy. Their privacy guarantee protects only against a specific class of adversaries. The error of the approximate answer returned by their algorithm is large --- the magnitude of noise grows exponentially with the number of edges in the subgraph. In~\cite{DBLP:conf/stoc/NissimRS07} and \cite{DBLP:journals/pvldb/KarwaRSY11}, $k$-triangle and $k$-star counting are studied, and they achieve better privacy and utility guarantee. In particular, they achieve $\epsilon$-differential privacy for $k$-star counting, and $(\epsilon,\delta)$-differential privacy, a weaker version of differential privacy, for $k$-triangle counting. However, their work cannot be extended to other kinds of subgraph. It is also worthy of mention the work in \cite{DBLP:conf/icdm/HayLMJ09}, which gives an algorithm for releasing an approximation to the degree distribution
of a graph and achieves $k$-edge differential privacy.

A major problem of the above work is that they can only achieve edge privacy --- each edge corresponds to a participant to be protected. But for many real-world data, such as social networks, each individual participant contributes to the graph a node rather than just an edge. We desire privacy protection based on nodes rather than edges. Unfortunately, it is difficult to achieve node differential privacy while obtaining reasonable query accuracy, because the maximum possible change to the query answer resulted from the change of one node~(as well as all of its incident edges) is comparable to the graph size. Prior to our work, whether any nontrivial graph statistics can be released under node differential privacy with reasonable accuracy is still an open problem~\cite{DBLP:journals/pvldb/KarwaRSY11}. It was widely believed that algorithms achieving node differential privacy can only return query answers that are too noisy for practical applications~\cite{DBLP:conf/sigmod/KiferM11,DBLP:conf/icdm/HayLMJ09}. In this paper, we try to challenge this seemingly impossible task and give a general solution.

In reality, databases usually consist of a number of tables. A participant may contribute tuples to several tables, and a tuple can be contributed collectively by multiple participants. A user may want to issue a SQL query to the database to obtain an output table, then requests approximate statistic of the output table. Subgraph counting is, in fact, a special case of this general context, because every subgraph count can be written as a SELECT query. It will be quite useful if this kind of task can be solved under differential privacy. There have been at least two attempts in the literature~\cite{DBLP:conf/sigmod/McSherry09,Palamidessi12}, which are based on bounding the \emph{global sensitivity} of the query. However, these works support only restricted kinds of join operations, where one participant can affect only constant number of tuples in the output table. Even the most simple subgraph counting requires unrestricted joins where a participant can have unbounded impact on the query answer. Obviously, existing methods are unable to support this kind of joins.

We focuses on the case where the SQL query can be translated into a series of positive relational algebra calculation. We aim at releasing an approximation to a linear statistic of the output table with reasonable accuracy under differential privacy. Our solution covers subgraph counting. Both node and edge differential privacy are achievable, depending on the choice of user. Node differential privacy is stronger than edge differential privacy, but the latter can allow better query accuracy. When nodes or edges of the graph are associated with auxiliary information, our solution also allows arbitrary kinds of constraints imposed on any edges or nodes of the subgraph, which are not supported by prior works.

\subsection{Contributions and Organization}

To develop differentially private mechanisms that can support unrestricted joins, we are in the face of several difficulties. First, the problem we study allows one participant to have complex impact on the database. The data model assumed by existing differentially private studies, in which each record corresponds to a unique participant, is too simple to suffice our need to express the complex relations between the database and the participants. Hence, new data model is needed to express how participants affect the database content.

Second, existing notions of \emph{sensitivity}, such as global and local sensitivity, are no longer appropriate in our case, because a new participant joining the database can, in the worst case, have unlimited impact on the query answer, leading to unbounded sensitivity. Thus, it is impossible for us to calibrate the noise to such sensitivities. We need a new metric to measure the least magnitude of noise that is necessary to answer a query.

Prior work for complex queries often compromise privacy guarantee, utility guarantee or efficiency guarantee. However, such comprises can lead to severe problem for practical use, which limit the applications of those techniques. It is a very challenging task to develop mechanism that can achieve all three guarantees.

Our contributions can be summarized into following

1) We propose a very general model of sensitive databases, which allows one participant to affect the database content in any possible way. Via formalizing the definition of neighborhood, the notion of differential privacy on this data model is setting up such that privacy protection is based on individual participants.

2) We propose a new notion of sensitivity, called \emph{empirical sensitivity}, which measures the maximum possible change to the query answer when a participant withdraws its data from the current database content. Empirical sensitivity is always bounded, and is often small. It gives a better measure of the least magnitude of noise that is necessary to answer a query.

3) We develop a general but inefficient mechanism to answer any monotonic query on a sensitive database. This mechanism guarantees $\epsilon$-differential privacy, and the error bound is roughly proportional to the \emph{global empirical sensitivity} of the query.

4) We propose a more special data model based on $K$-relation or $c$-table, a notion that comes from the field of uncertain databases. Every tuple in a $K$-relation is annotated with a positive Boolean expression that specifies its condition of presence. $K$-relation is closed under positive relational algebra calculation, hence it can be used to express the complex relations between the participants and the table output by a SQL query.

5) We develop an efficient mechanism to answer any linear query to a sensitive $K$-relation. This mechanism guarantees $\epsilon$-differential privacy, and the error bound is roughly proportional to the \emph{universal empirical sensitivity} of the query. The computation cost is in a polynomial of the size of $K$-relation. This mechanism also implies the first solution to the problem of subgraph counting for any subgraphs, which can achieve either node differential privacy or edge differential privacy, and the error bound is roughly proportional to the \emph{local empirical sensitivity} of the query.

In Fig.~\ref{fig:intro:compare} we present a brief comparison between our work and prior work.

\begin{figure*}[!t]
    \centering
    \begin{tabular}{|m{0.32\textwidth}|m{0.3\textwidth}|m{0.32\textwidth}|}
    \hline
    Queries & Our mechanism & Existing mechanisms \\\hline
    Monotonic query on a sensitive database &
    $\widetilde{O}(\widetilde{GS}_q/\epsilon)$ error, $\EXP(|P|)$ time &
    None \\\hline

    Linear statistic of the output of a SQL query &
    $\widetilde{O}(\widetilde{US}_q/\epsilon)$ error, $\POLY(|P|,|R|)$ time &
    \parbox{.32\textwidth}{$O(US_q/\epsilon)$ error and $O(1)$ time if there are no unrestricted joins~\cite{DBLP:conf/sigmod/McSherry09,Palamidessi12}\\ Not solvable if there are unrestricted joins because $US_q\geq GS_q=+\infty$} \\\hline

    triangle counting (\includegraphics[height=10pt]{intro/triangle}) &
    $\widetilde{O}(\widetilde{LS}_q/\epsilon)$ error, $\POLY(k,|R|)$ time &
    $O(LS_q/\epsilon+1/\epsilon^2)$ error; $O(|V|\cdot|E|)$ time; only achieve differential privacy based on edges~\cite{DBLP:conf/stoc/NissimRS07} \\\hline

    $k$-star counting (e.g., 3-star \includegraphics[height=10pt]{intro/k-star}) &
    $\widetilde{O}(\widetilde{LS}_q/\epsilon)$ error, $\POLY(k,|R|)$ time or $\POLY(|V|,|E|,k)$ time &
    $O(LS_q/\epsilon)$ error if $1/\epsilon=O(d_{\max}/k)$; $O(|V|\cdot|E|)$ time; only achieve differential privacy based on edges~\cite{DBLP:journals/pvldb/KarwaRSY11} \\\hline

    $k$-triangle counting (e.g., 3-triangle \includegraphics[height=10pt]{intro/k-triangle}) &
    $\widetilde{O}(\widetilde{LS}_q/\epsilon)$ error, $\POLY(k,|R|)$ time or $\POLY(|V|,|E|,k)$ time &
    $O(LS_q/\epsilon)$ error if $\ln(1/\delta)/\epsilon=O(a_{\max})$; $O(|V|\cdot|E|)$ time; only achieve $(\epsilon,\delta)$-differential privacy based on edges~\cite{DBLP:journals/pvldb/KarwaRSY11} \\\hline

    $k$-node $l$-edge connected subgraph counting &
    $\widetilde{O}(\widetilde{LS}_q/\epsilon)$ error, $\POLY(k,l,|R|)$ time &
    $\Theta((k l^2\log |V|)^{l-1}/\epsilon)$ error; $O(1)$ time; only achieve adversary privacy based on edges w.r.t. a specific class of adversaries~\cite{DBLP:conf/pods/RastogiHMS09} \\\hline

    \end{tabular}

    \caption{Comparison between our mechanism and existing mechanisms. $\widetilde{O}$ means that logarithmic factors are omitted. For sensitive database, $|P|$ denotes the number of participants and $|\SUPP(R)|$ denotes the number of tuples returned by the SQL query. For subgraph counting, $|V|$ and $|E|$ denote the number of nodes and edges in the graph, and $|R|=|\SUPP(R)|$ denotes the true query answer. $d_{\max}$ denotes the maximum degree of a node, and $a_{\max}$ denotes the maximum number of common neighbors of a pair of nodes. $GS$, $LS$, $US$, $\widetilde{GS}$, $\widetilde{LS}$ and $\widetilde{US}$ are explained in Sec.~\ref{sec:pre} and Sec.~\ref{sec:problem}. We have $\widetilde{LS}_q\leq LS_q$ and $\widetilde{US}_q\leq US_q$. Note that we do not take account of the time needed for generating the output table or the list of matched subgraphs in the computation cost. For subgraph counting our solution can achieve differential privacy based on either nodes or edges, depending on the choice of user.}
    \label{fig:intro:compare}
\end{figure*}

